Solving Deep Reinforcement Learning Tasks with Evolution Strategies and Linear Policy Networks

Although deep reinforcement learning methods can learn effective policies for challenging problems such as Atari games and robotics tasks, algorithms are complex, and training times are often long. This study investigates how Evolution Strategies perform compared to gradient-based deep reinforcement learning methods. We use Evolution Strategies to optimize the weights of a neural network via neuroevolution, performing direct policy search. We benchmark both deep policy networks and networks consisting of a single linear layer from observations to actions for three gradient-based methods, such as Proximal Policy Optimization. These methods are evaluated against three classical Evolution Strategies and Augmented Random Search, which all use linear policy networks. Our results reveal that Evolution Strategies can find effective linear policies for many reinforcement learning benchmark tasks, unlike deep reinforcement learning methods that can only find successful policies using much larger networks, suggesting that current benchmarks are easier to solve than previously assumed. Interestingly, Evolution Strategies also achieve results comparable to gradient-based deep reinforcement learning algorithms for higher-complexity tasks. Furthermore, we find that by directly accessing the memory state of the game, Evolution Strategies can find successful policies in Atari that outperform the policies found by Deep Q-Learning. Evolution Strategies also outperform Augmented Random Search in most benchmarks, demonstrating superior sample efficiency and robustness in training linear policy networks.

==> IJCAI24_submission/latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> IJCAI24_submission/old_tables.tex <==


% \begin{table}[htbp]
%     \centering
%     \caption{Mean and standard deviation of the best average episodic return on MuJoCo environments averaged over five random seeds.}
%     \label{tab:mujoco_performance}
%     \scriptsize
%     \setlength\tabcolsep{2pt}
%     \begin{tabular}{lcccccc}
%         \toprule
%         Algorithm & \multicolumn{1}{c}{Hopper} & \multicolumn{1}{c}{Walker2D} & \multicolumn{1}{c}{HalfCheetah} & \multicolumn{1}{c}{Ant} & \multicolumn{1}{c}{Swimmer} & \multicolumn{1}{c}{Humanoid} \\
%         \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
%         & M(SD) & M(SD) & M(SD) & M(SD) & M(SD) & M(SD) \\
%         \midrule
%         PPO & 2955 (1108) & 4237 (302) & 2651 (1260) & 3378 (510) & 110 (27) & 980 (533) \\
%         PPO Linear & 1050 (463) & 738 (396) & 2291 (1477) & 3542 (350) & 35 (10) & 922 (361)\\
%         SAC &  3614 (81) & 4731 (444) & 14534 (388) & 6059 (639) & 71 (34) & 6342 (127) \\
%         SAC Linear & 168 (73) & 361 (54) & -98 (165) & -22 (38) & 29 (6) & 757 (403) \\
%         CSA & ...(...) & ...(...) & ... & ... & ... & ... \\
%         CMA-ES & ...(...) & ...(...) & ... & ... & ... & ... \\
%         sep-CMA-ES & ...(...) & ...(...) & ... & ... & ... & ... \\
%         \bottomrule
%     \end{tabular}
% \end{table}


% \begin{table}[htbp]
%     \centering
%     \caption{Mean (M) and standard deviation (SD) of the best average episodic return on Classic Control environments averaged over ten random seeds trained over 500,000 timesteps.}
%     \label{tab:atari_performance}
%     \begin{tabular}{lccc}
%         \toprule
%         & \multicolumn{1}{c}{CartPole} & \multicolumn{1}{c}{Pendulum} & \multicolumn{1}{c}{Acrobot} \\
%         \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
%         Algorithm & M (SD) & M (SD) & M (SD) \\
%         \midrule
%         PPO & 500 (0) & -874 (229) & ... \\
%         PPO Linear & 223 (133) & -984 (133) & -133 (31) \\
%         DQN & 500 (0) & - & -76 (8) \\
%         DQN Linear & 40 (20) & - & -96 (35) \\
%         SAC & - & -39 (57) & - \\
%         SAC Linear & - & -1035 (221) & - \\
%         CSA & 500 (0) & -670 (61) & -69 (1.0)  \\
%         CMA-ES & 500 (0) & -668 (81) & -69 (1.0) \\
%         sep-CMA-es & 500 (0) & -681 (82) & -70 (1) \\
%         \bottomrule
%     \end{tabular}
% \end{table}









% \begin{table}[htbp]
%     \centering
%     \caption{Mean and standard deviation of the best average episodic return on Box2D environments averaged over five random seeds trained over 500,000 timesteps.\jacob{If you add more timesteps for walker it solves for es}}
%     \label{tab:box2d_performance}
%     \begin{tabular}{lcc}
%         \toprule
%         & \multicolumn{1}{c}{Lunarlander} & \multicolumn{1}{c}{Bipedalwalker} \\
%         \cmidrule(lr){2-2} \cmidrule(lr){3-3}
%         Algorithm & M(SD) & M(SD) \\
%         \midrule
%         PPO & 114 (96) & 286 (7) \\
%         PPO Linear & -32 (34) & 225 (35) \\
%         DQN & 240 (21) & - \\
%         DQN Linear & -52 (46) & - \\
%         SAC & - & 264 (113) \\
%         SAC Linear & - & -70 (23) \\
%         CSA & 250 (89) & -11 (88) \\
%         CMA-ES & 273 (8) & -54 (36) \\
%         sep-CMA-ES & 273 (8) & -25 (55) \\
%         \bottomrule
%     \end{tabular}

\clearpage
\onecolumn

\begin{longtable}{lrlrrrrr} 
% \caption{Descriptory statistics for the maximum episodic return computed over \textit{`count'} trials for each of benchmarks considered, with \textit{`n\_timesteps'} used to train each method.}
\toprule
env & n\_timesteps & method & count & min & mean & max & std \\
\midrule
\endfirsthead
\toprule
env & n\_timesteps & method & count & min & mean & max & std \\
\midrule
\endhead
\midrule
\multicolumn{8}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Swimmer-v4 & 1.00e+06 & cma-es & 10 & 2.67e+02 & 3.51e+02 & 3.62e+02 & 2.96e+01 \\
Swimmer-v4 & 1.00e+06 & csa & 10 & 3.58e+02 & 3.61e+02 & 3.62e+02 & 1.29e+00 \\
Swimmer-v4 & 1.00e+06 & ppo large & 5 & 5.11e+01 & 9.89e+01 & 1.19e+02 & 2.72e+01 \\
Swimmer-v4 & 1.00e+06 & ppo small & 5 & 1.93e+01 & 3.53e+01 & 4.45e+01 & 1.04e+01 \\
Swimmer-v4 & 1.00e+06 & sac large & 5 & 4.78e+01 & 5.08e+01 & 5.55e+01 & 2.90e+00 \\
Swimmer-v4 & 1.00e+06 & sac small & 7.00e+00 & 2.53e+01 & 3.29e+01 & 3.52e+01 & 3.37e+00 \\
Swimmer-v4 & 1.00e+06 & sep-cma-es & 10 & 1.83e+02 & 3.42e+02 & 3.61e+02 & 5.57e+01 \\ \hline
Hopper-v4 & 1.00e+06 & cma-es & 10 & 2.62e+03 & 2.88e+03 & 3.13e+03 & 1.81e+02 \\
Hopper-v4 & 1.00e+06 & csa & 10 & 2.68e+03 & 2.96e+03 & 3.14e+03 & 1.29e+02 \\
Hopper-v4 & 1.00e+06 & ppo large & 5 & 1.00e+03 & 2.94e+03 & 3.54e+03 & 1.09e+03 \\
Hopper-v4 & 1.00e+06 & ppo small & 5 & 7.15e+02 & 9.11e+02 & 1.25e+03 & 2.20e+02 \\
Hopper-v4 & 1.00e+06 & sac large & 5 & 3.55e+03 & 3.62e+03 & 3.72e+03 & 7.61e+01 \\
Hopper-v4 & 1.00e+06 & sac small & 10 & 1.27e+02 & 1.39e+02 & 1.55e+02 & 1.31e+01 \\
Hopper-v4 & 1.00e+06 & sep-cma-es & 10 & 1.42e+03 & 2.72e+03 & 2.97e+03 & 4.68e+02 \\ \hline
HalfCheetah-v4 & 1.00e+06 & cma-es & 10 & 1.92e+03 & 3.50e+03 & 4.64e+03 & 8.20e+02 \\
HalfCheetah-v4 & 1.00e+06 & csa & 10 & 2.12e+03 & 3.50e+03 & 4.24e+03 & 7.85e+02 \\
HalfCheetah-v4 & 1.00e+06 & ppo large & 5 & 1.49e+03 & 2.21e+03 & 3.70e+03 & 9.25e+02 \\
HalfCheetah-v4 & 1.00e+06 & ppo small & 5 & 1.08e+03 & 1.96e+03 & 3.45e+03 & 1.16e+03 \\
HalfCheetah-v4 & 1.00e+06 & sac large & 5 & 1.15e+04 & 1.17e+04 & 1.19e+04 & 1.81e+02 \\
HalfCheetah-v4 & 1.00e+06 & sac small & 5 & 8.43e+00 & 9.19e+01 & 1.98e+02 & 7.27e+01 \\
HalfCheetah-v4 & 1.00e+06 & sep-cma-es & 10 & 2.75e+03 & 3.43e+03 & 4.39e+03 & 6.39e+02 \\ \hline
Walker2d-v4 & 1.00e+06 & cma-es & 10 & 5.63e+02 & 1.96e+03 & 3.03e+03 & 8.98e+02 \\
Walker2d-v4 & 1.00e+06 & csa & 10 & 5.11e+02 & 1.66e+03 & 3.20e+03 & 9.41e+02 \\
Walker2d-v4 & 1.00e+06 & ppo large & 5 & 3.96e+03 & 4.24e+03 & 4.54e+03 & 2.62e+02 \\
Walker2d-v4 & 1.00e+06 & ppo small & 5 & 4.27e+02 & 6.73e+02 & 8.86e+02 & 1.98e+02 \\
Walker2d-v4 & 1.00e+06 & sac large & 5 & 4.14e+03 & 4.78e+03 & 5.25e+03 & 5.18e+02 \\
Walker2d-v4 & 1.00e+06 & sac small & 5 & 3.29e+02 & 3.39e+02 & 3.55e+02 & 1.08e+01 \\
Walker2d-v4 & 1.00e+06 & sep-cma-es & 10 & 6.94e+02 & 2.10e+03 & 2.73e+03 & 6.78e+02 \\ \hline
Ant-v4 & 1.00e+07 & cma-es & 10 & 2.26e+03 & 2.82e+03 & 3.51e+03 & 3.73e+02 \\
Ant-v4 & 1.00e+07 & csa & 10 & 2.37e+03 & 2.73e+03 & 3.19e+03 & 2.77e+02 \\
Ant-v4 & 1.00e+07 & ppo large & 5 & 2.95e+03 & 3.39e+03 & 4.20e+03 & 5.04e+02 \\
Ant-v4 & 1.00e+07 & ppo small & 5 & 3.19e+03 & 3.54e+03 & 4.13e+03 & 3.54e+02 \\
Ant-v4 & 1.00e+07 & sac large & 5 & 5.19e+03 & 6.20e+03 & 6.74e+03 & 5.94e+02 \\
Ant-v4 & 1.00e+07 & sac small & 3.00e+00 & -2.00e+01 & -1.72e+01 & -1.27e+01 & 3.92e+00 \\
Ant-v4 & 1.00e+07 & sep-cma-es & 10 & 1.96e+03 & 2.68e+03 & 3.46e+03 & 4.69e+02 \\ \hline
Humanoid-v4 & 1.00e+07 & csa & 10 & 6.87e+02 & 8.22e+02 & 9.71e+02 & 7.87e+01 \\
Humanoid-v4 & 1.00e+07 & ppo large & 5 & 7.10e+02 & 8.15e+02 & 9.34e+02 & 9.00e+01 \\
Humanoid-v4 & 1.00e+07 & ppo small & 5 & 7.78e+02 & 7.92e+02 & 8.11e+02 & 1.44e+01 \\
Humanoid-v4 & 1.00e+07 & sac large & 5 & 6.27e+03 & 6.51e+03 & 6.69e+03 & 1.61e+02 \\
Humanoid-v4 & 1.00e+07 & sac small & 5 & 5.84e+02 & 6.04e+02 & 6.30e+02 & 1.77e+01 \\
Humanoid-v4 & 1.00e+07 & sep-cma-es & 10 & 6.84e+02 & 8.30e+02 & 1.03e+03 & 1.04e+02 \\ \hline
LunarLander-v2 & 5.00e+05 & cma-es & 10 & 2.58e+02 & 2.73e+02 & 2.84e+02 & 7.58e+00 \\
LunarLander-v2 & 5.00e+05 & csa & 10 & 8.45e-02 & 2.50e+02 & 2.93e+02 & 8.87e+01 \\
LunarLander-v2 & 5.00e+05 & dqn large & 5 & 2.31e+02 & 2.51e+02 & 2.76e+02 & 1.70e+01 \\
LunarLander-v2 & 5.00e+05 & dqn small & 5 & -1.83e+01 & -8.84e+00 & 9.54e+00 & 1.12e+01 \\
LunarLander-v2 & 5.00e+05 & ppo large & 5 & 6.65e+01 & 1.25e+02 & 1.95e+02 & 6.32e+01 \\
LunarLander-v2 & 5.00e+05 & ppo small & 5 & -6.86e+01 & -4.67e+01 & -3.46e+01 & 1.30e+01 \\
LunarLander-v2 & 5.00e+05 & sep-cma-es & 10 & 2.57e+02 & 2.73e+02 & 2.91e+02 & 1.02e+01 \\ \hline
BipedalWalker-v3 & 2.00e+06 & cma-es & 10 & 1.61e+02 & 2.38e+02 & 3.01e+02 & 5.03e+01 \\
BipedalWalker-v3 & 2.00e+06 & csa & 10 & 1.64e+02 & 2.29e+02 & 3.01e+02 & 4.93e+01 \\
BipedalWalker-v3 & 2.00e+06 & ppo large & 5 & 2.79e+02 & 2.85e+02 & 2.95e+02 & 6.07e+00 \\
BipedalWalker-v3 & 2.00e+06 & ppo small & 5 & 1.58e+02 & 2.18e+02 & 2.60e+02 & 5.16e+01 \\
BipedalWalker-v3 & 2.00e+06 & sac large & 5 & 5.56e+01 & 2.65e+02 & 3.22e+02 & 1.17e+02 \\
BipedalWalker-v3 & 2.00e+06 & sac small & 5 & -1.00e+02 & -9.82e+01 & -9.38e+01 & 2.66e+00 \\
BipedalWalker-v3 & 2.00e+06 & sep-cma-es & 10 & 5.88e+01 & 1.91e+02 & 2.47e+02 & 5.97e+01 \\ \hline
Acrobot-v1 & 5.00e+05 & cma-es & 10 & -7.10e+01 & -6.87e+01 & -6.80e+01 & 9.44e-01 \\
Acrobot-v1 & 5.00e+05 & csa & 10 & -7.20e+01 & -6.95e+01 & -6.65e+01 & 1.42e+00 \\
Acrobot-v1 & 5.00e+05 & dqn large & 10 & -6.90e+01 & -6.51e+01 & -6.10e+01 & 3.24e+00 \\
Acrobot-v1 & 5.00e+05 & dqn small & 10 & -1.13e+02 & -7.70e+01 & -6.95e+01 & 1.44e+01 \\
Acrobot-v1 & 5.00e+05 & ppo large & 1.30e+01 & -7.15e+01 & -6.96e+01 & -6.40e+01 & 1.89e+00 \\
Acrobot-v1 & 5.00e+05 & ppo small & 1.30e+01 & -2.08e+02 & -1.34e+02 & -1.00e+02 & 3.70e+01 \\
Acrobot-v1 & 5.00e+05 & sep-cma-es & 10 & -7.25e+01 & -6.97e+01 & -6.80e+01 & 1.47e+00 \\ \hline
CartPole-v1 & 5.00e+05 & cma-es & 10 & 5.00e+02 & 5.00e+02 & 5.00e+02 & 0.00e+00 \\
CartPole-v1 & 5.00e+05 & csa & 10 & 5.00e+02 & 5.00e+02 & 5.00e+02 & 0.00e+00 \\
CartPole-v1 & 5.00e+05 & dqn large & 10 & 5.00e+02 & 5.00e+02 & 5.00e+02 & 0.00e+00 \\
CartPole-v1 & 5.00e+05 & dqn small & 10 & 1.20e+01 & 1.78e+01 & 5.30e+01 & 1.26e+01 \\
CartPole-v1 & 5.00e+05 & ppo large & 10 & 5.00e+02 & 5.00e+02 & 5.00e+02 & 0.00e+00 \\
CartPole-v1 & 5.00e+05 & ppo small & 10 & 1.32e+02 & 1.98e+02 & 2.60e+02 & 3.60e+01 \\
CartPole-v1 & 5.00e+05 & sep-cma-es & 10 & 5.00e+02 & 5.00e+02 & 5.00e+02 & 0.00e+00 \\ \hline
Pendulum-v1 & 5.00e+05 & cma-es & 10 & -8.83e+02 & -6.68e+02 & -6.26e+02 & 8.11e+01 \\
Pendulum-v1 & 5.00e+05 & csa & 10 & -8.09e+02 & -6.70e+02 & -6.28e+02 & 6.15e+01 \\
Pendulum-v1 & 5.00e+05 & ppo large & 10 & -1.01e+03 & -8.05e+02 & -6.29e+02 & 1.65e+02 \\
Pendulum-v1 & 5.00e+05 & ppo small & 10 & -1.09e+03 & -9.55e+02 & -8.70e+02 & 6.84e+01 \\
Pendulum-v1 & 5.00e+05 & sac large & 10 & -1.70e+02 & -1.26e+02 & -1.18e+02 & 1.56e+01 \\
Pendulum-v1 & 5.00e+05 & sac small & 10 & -1.12e+03 & -1.06e+03 & -9.39e+02 & 5.35e+01 \\
Pendulum-v1 & 5.00e+05 & sep-cma-es & 10 & -8.76e+02 & -6.81e+02 & -6.30e+02 & 8.16e+01 \\ \hline
SpaceInvaders-v5 & 5.00e+07 & cma-es & 10 & 1.47e+03 & 1.88e+03 & 2.42e+03 & 3.27e+02 \\
SpaceInvaders-v5 & 5.00e+07 & csa & 10 & 8.30e+02 & 1.62e+03 & 2.64e+03 & 5.58e+02 \\
SpaceInvaders-v5 & 5.00e+07 & sep-cma-es & 10 & 1.20e+03 & 1.49e+03 & 1.74e+03 & 1.91e+02 \\ \hline
Atlantis-v5 & 5.00e+07 & cma-es & 10 & 6.56e+04 & 8.71e+04 & 1.04e+05 & 1.09e+04 \\
Atlantis-v5 & 5.00e+07 & csa & 10 & 6.18e+04 & 8.44e+04 & 1.01e+05 & 1.29e+04 \\
Atlantis-v5 & 5.00e+07 & sep-cma-es & 10 & 7.67e+04 & 8.86e+04 & 9.95e+04 & 9.12e+03 \\ \hline
\end{longtable}

==> biographies.tex <==
\begin{document}

\section*{Biography Section}

\begin{IEEEbiographynophoto}{Annie Wong}
Annie Wong is a PhD candidate at the Natural Computing Group at the Leiden Institute of Advanced Computer Science (LIACS) and a data scientist in Industry Solutions Engineering (ISE) at Microsoft. Her research is dedicated to the interdisciplinary field of evolutionary algorithms and reinforcement learning to solve complex optimization problems. She aims to use these advanced computational techniques to develop innovative solutions to address challenges in both research and practical applications.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jacob de Nobel}
Biography text here without a photo.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Thomas B\"ack} (M’95-SM’19-F’22)
 is Full Professor of Computer Science at the Leiden Institute of Advanced Computer Science (LIACS), Leiden University, The Netherlands, since 2002. 
 He received the Diploma degree in computer science in 1990 and the PhD~degree in 1994, both from the University of Dortmund, Germany. 
 His research interests include evolutionary computation, machine learning, and their real-world applications, especially in sustainable smart industry and health.

 Prof.~B\"ack’s awards and honors include membership in the Royal Netherlands Academy of Arts and Sciences (KNAW, 2021) and Academia Europaea (2022), the IEEE Computational Intelligence Society Evolutionary Computation Pioneer Award (2015), Fellow of the International Society of Genetic and Evolutionary Computation (2003), and best Ph.D.~thesis award of the German society of Computer Science (GI, 1995).
 
 He currently serves as an Editor in Chief for MIT Press's Evolutionary Computation Journal, Associate Editor for the IEEE Transactions on Evolutionary Computation and Artificial Intelligence Review journals, and as area editor for the ACM Transactions on Evolutionary Learning and Optimization. He is co-editor of the Natural Computing Book Series, Handbook of Evolutionary Computation, Handbook of Natural Computing, and author of Evolutionary Computation in Theory and Practice. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Aske Plaat}
Aske Plaat is professor in artificial intelligence at Leiden University and heads the Sustainable Energy Learning Lab and the Reinforcement Learning Group. He is the author of two textbooks on Deep Reinforcement Learning. His research interests are in reinforcement learning and self-learning systems. He has won the Novag Award for the best computer chess publication. He is co-author of an ERC Advanced grant on combinatorial algorithms for high energy physics. From 2016-2023 he served two terms as scientific director of the institute of artificial intelligence and computer science LIACS. Previously he has worked at the Vrije Universiteit Amsterdam, Tilburg University, the University of Alberta, and the Massachusetts Institute of Technology.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Anna V. Kononova}
(M'04) is Assistant Professor in Efficient Heuristic Optimisation at the Leiden Institute of Advanced Computer Science. She received her MSc degree in Applied Mathematics from Yaroslavl State University in 2004 and her PhD degree in Computer Science from University of Leeds in 2010. After her postdoctoral experiences at Technical University Eindhoven and Heriot-Watt University, Anna spent 5 years working as an engineer and a mathematician in industry. Her current research interests include analysis of behaviour of optimisation algorithms and machine learning.
\end{IEEEbiographynophoto}

\end{document}
